Deep Distributional Learning with Non-crossing Quantile Network

In this paper, we introduce a non-crossing quantile (NQ) network for conditional distribution learning. By leveraging non-negative activation functions, the NQ network ensures that the learned distributions remain monotonic, effectively addressing the issue of quantile crossing. Furthermore, the NQ network-based deep distributional learning framework is highly adaptable, applicable to a wide range of applications, from classical non-parametric quantile regression to more advanced tasks such as causal effect estimation and distributional reinforcement learning (RL). We also develop a comprehensive theoretical foundation for the deep NQ estimator and its application to distributional RL, providing an in-depth analysis that demonstrates its effectiveness across these domains. Our experimental results further highlight the robustness and versatility of the NQ network.

==> figures/Theory.tex <==

\section{Learning Guarantees}\label{sec_theory}

In this section, we prove the consistency and derive non-asymptotic upper bounds for the proposed NQ network estimator. Recall  the target $Q_Y$ minimizes the risk $\mathcal{L}$, thus $\mathcal{L}(Q_Y)\le \mathcal{L}(f)$ for any estimator $f$. We define its excess risk by
\begin{align}\label{excess_risk}
    \mathcal{R}(f):=\mathcal{L}(f)-\mathcal{L}(Q_Y).
\end{align}
 We %then intend to 
 aim to derive non-asymptotic upper bounds for $\mathcal{R}(\hat{f}_N)$, i.e., the excess risk of the proposed empirical risk minimizer $\hat{f}_N$ defined in (\ref{erm}). It is worth noting that under proper conditions, the convergence of excess risk $\mathcal{R}(\hat{f}_N)$ toward zero implies the convergence of the estimator $\hat{f}_N$ towards the target $Q_Y$. We elucidate this in section \ref{sec_selfcali}. Let $\mathcal{R}_N(f):=\mathcal{L}_N(f)-\mathcal{L}_N(Q_Y)$ denote the empirical version of the excess risk, we first give preliminary bounds on the excess risks based on error decomposition.
\begin{lemma}\label{decomposition}
    The excess risk $\mathcal{R}(\hat{f}_N)$ of the empirical risk minimizer $\hat{f}_N$ defined in (\ref{erm}) satisfies
    $\mathbb{E}[\mathcal{R}(\hat{f}_N)]\le \mathbb{E}[\mathcal{R}(\hat{f}_N)-2\mathcal{R}_N(\hat{f}_N)] +2\inf_{f\in\mathcal{F}_N}\mathcal{R}(f),$
    where $\mathbb{E}[\mathcal{R}(\hat{f}_N)-2\mathcal{R}_N(\hat{f}_N)]$ is called the {\it variance} or {\it stochastic error} and $2\inf_{f\in\mathcal{F}_N}[\mathcal{R}(f)]$ is called the {\it bias} or {\it approximation error}.
\end{lemma}

The {\it bias} or the {\it approximation error} measures the distance between the regression functions (hypothesis class) $\mathcal{F}_N$ and the target function $Q_Y$. The {\it bias} is closely related to the expressiveness power of the hypothesis class of NQ networks $\mathcal{F}_N$ and the properties of the target function $Q_Y$, e.g., its structure, continuity, and smoothness. In general, richer classes of $\mathcal{F}_N$ and simpler target functions $Q
_Y$ leads to smaller {\it bias}. It is worth noting that, most parametric methods assume the model is correctly specified in the sense that the target $Q_Y$ belongs to the hypothesis class $\mathcal{F}_N$. In that case, the {\it bias} or the {\it approximation error} $\inf_{f\in\mathcal{F}_N}\mathcal{R}(f)$ is zero, and the convergence of the estimator turns out to have ``parametric rate".

The {\it variance} or {\it stochastic error} measure the estimation error induced by the randomness of the sampling.  It is closely related to the loss function, the sample size, and the properties of the hypothesis class $\mathcal{F}_N$. In general, the smaller sample size of $N$ and richer class of $\mathcal{F}_N$ lead to greater {\it variance}. The {\it variance} can be analyzed using empirical process theories based on neural network complexity analysis \citep{anthony1999,bartlett2019nearly}. 


\subsection{Non-asymptotic error bounds without misspecification}
In this subsection, we assume the model is correctly specified (the target $ Q_Y \in\mathcal{F}_N$) and derive non-asymptotic upper bounds for the excess risks of NQ-net estimations. With correctly specified model assumption, the {\it bias} term $\inf_{f\in\mathcal{F}_N}\mathcal{R}(f)$ in the excess risk bound in Lemma (\ref{decomposition}) disappears. Then it suffices to analyze the upper bound of the {\it variance} or {\it stochastic error} to obtain an upper bound of excess risk of the NQ net estimator $\hat{f}_N$ defined in (\ref{erm}).

\begin{theorem}\label{sto_error}
    Let the classes of neural networks $\mathcal{F}_N$ be defined as in section \ref{sec_training} with depth $\mathcal{D}$, size $\mathcal{S}$ and bound $\mathcal{B}$, and the excess risk $\mathcal{R}$ be defined as in (\ref{excess_risk}), and suppose the target quantile curves $Q_Y=(Q_Y^{\tau_1},\ldots,Q_Y^{\tau_K})\in\mathcal{F}_N$. Then the NQ net estimator $\hat{f}_N$ defined in (\ref{erm}) satisfies
\begin{align}\notag
    &\mathbb{E}[\mathcal{R}(\hat{f}_N)]\le C\cdot K\mathcal{B}^3\frac{\mathcal{S}\mathcal{D}\log(\mathcal{S})\log(N)}{N},
\end{align}
for $N\ge C_0\mathcal{S}\mathcal{D}\log \mathcal{S}$ where $C, C_0>0$ are universal constants. %$\mathcal{S}$ and $\mathcal{D}$ denote the size (total number of parameters) and depth of the NQ networks in $\mathcal{F}_N$.
\end{theorem}

The excess risk bound in Theorem \ref{sto_error} %obtains a non-asymptotic bound of the excess risk of the NQ network estimator when the model is correctly specified, i.e., the target function $Q_Y\in\mathcal{F}_N$.  
has an order $O({\mathcal{S}\mathcal{D}\log(\mathcal{S})\log(N)}{N}^{-1})$, which decreases in the sample size $N$ linearly and increases in the network complexity (size and depth) linearly. It is worth noting that the rate in Theorem \ref{sto_error} is squarely faster than $O(\sqrt{{\mathcal{S}\mathcal{D}\log(\mathcal{S})\log(N)}{N}^{-1}})$ derived from standard concentration inequality for deep quantile networks \citep{padilla2022quantile,shen2024nonparametric} and other nonparametric methods \citep{takeuchi2006nonparametric,sangnier2016joint,mohri2018foundations}.

Under calibration conditions (see Lemma \ref{calib} in Appendix \ref{sec_selfcali}), the convergence of the excess risk also implies the convergence of the NQ network estimator towards the target function in the sense that $\sum_{k=1}^K\mathbb{E}\vert \hat{f}^{\tau_k}_{N}(X)-Q_Y^{\tau_k}(X)\vert^2\le C^\prime\cdot K\mathcal{B}^3{\mathcal{S}\mathcal{D}\log(\mathcal{S})\log(N)}{N}^{-1}$, which also implies that  ``parametric rate" $O(N^{-1})$ for the convergence of each conditional quantile estimate $\hat{f}^{\tau_k}_{N}$.


\begin{comment}
    \begin{lemma}[Stochastic Error bound]\label{sto_error}
    Let the classes of neural networks $\mathcal{F}_N$ be defined as in section \ref{sec_training}, and the excess risk $\mathcal{R}$ (empirical excess risk $\mathcal{R}_N$) be defined as in (\ref{excess_risk}), and suppose the target quantile curves $Q_Y=(Q_Y^{\tau_1},\ldots,Q_Y^{\tau_K})$ are bounded by $\mathcal{B}$. Then for any $\delta>0$, with probability at least $1-\delta$
\begin{align}\notag
    &\sup_{f\in\mathcal{F}_N}\vert \mathcal{R}(f)-\
    \mathcal{R}_N(f)\vert \le \frac{2\sqrt{2}(K+2)\mathcal{B})}{\sqrt{N}}\bigg(C\sqrt{K\mathcal{S}\mathcal{D}\log(\mathcal{S})\log(N)}+\sqrt{\log (1/\delta)}\bigg),
\end{align}
for $N\ge C_1\mathcal{S}\mathcal{D}\log \mathcal{S}$ where $C,C_1>0$ are universal constants.
\end{lemma}
\end{comment}



\subsection{Non-asymptotic error bound with misspecification}

For nonparametric regression, the target function can be complex and might not belong to the hypothesis class. In this case, the model is misspecified, leading to a nonzero bias or approximation error when using the hypothesis class to estimate the target function.

The {\it bias} or {\it approximation error} depends on the representational power of the hypothesis class $\mathcal{F}_N$ and the features of the target function $Q_Y$, e.g., its structure, continuity, and smoothness. Here, we introduce the concept of a general class of functions, i.e., H\"older smooth functions to describe the smoothness feature of the target function and further quantify the approximation error. We assume that each component of the target $Q_Y=(Q_Y^{\tau_1}, \ldots, Q_Y^{\tau_K})$ is a H\"older smooth function. 

\begin{definition}\label{holder_function}
Given constants $B,\beta>0$, the H\"older class of functions $\mathcal{H}^\beta(\mathcal{X},B)$  is defined as
\begin{align}
\label{Hclass}
&\mathcal{H}^\beta(\mathcal{X},B) =
\Big\{f: \mathcal{X}\to\mathbb{R},\max_{\Vert\alpha\Vert_1\le s}\Vert\partial^\alpha f\Vert_\infty\le B,\max_{\Vert\alpha\Vert_1=s} \sup_{x\not=y}\frac{\vert\partial^\alpha f(x)-\partial^\alpha f(y)\vert}{\Vert x-y\Vert_2^r}\le B \Big\}, \nonumber
\end{align}
where $\partial^\alpha=\partial^{\alpha_1}\cdots\partial^{\alpha_d}$ with $\alpha=(\alpha_1,\ldots,\alpha_d)^\top\in\mathbb{N}_0^d$ and $\Vert\alpha\Vert_1=\sum_{i=1}^d\alpha_i$.
\end{definition}

The classes of Lipschitz continuous and continuously differentiable functions are  H\"older function classes. To analyze the {\it bias}, %in terms of the network approximation, without loss of generality, 
we make the following assumptions.

\begin{assumption}\label{assump1} 
(i) The target quantile curves $Q_Y=(Q_Y^{\tau_1},\ldots,Q_Y^{\tau_K})$ are $\beta$-H\"older smooth with constant $B$. (ii) The domain of the target function $Q_Y$ is $\mathcal{X}=[0,1]^d$. The probability distribution of covariate $X$ is absolutely continuous with respect to the Lebesgue measure.
\end{assumption}

%The (i) in 
Assumption \ref{assump1}(i) quantifies the smoothness %features 
of target quantile curves $Q_Y=(Q_Y^{\tau_1},\ldots, Q_Y^{\tau_K})$. The smoothness parameter $\beta$ %can be an indicator of
characterizes how difficult the target function can be approximated by the hypothesis class, and the approximation error depends directly on $\beta$ \citep{schmidt2020nonparametric,shen2019deep}. %The (ii) in 
Assumption \ref{assump1}(ii) is a regular condition %where in most scenarios of approximation theories the approximation is focused 
that restricts the covariate space to a bounded domain, which we set to $[0,1]^d$ without loss of generality. %we set the domain to . 
More generally, %although 
the range of the domain can be arbitrarily large.  %we are interested in the approximation result on $[0,1]^d$. 
Similar assumptions can be found in \cite{yarotsky2017error,petersen2018optimal,guhring2020error,jiao2023deep}.

\begin{lemma}[Approximation Error bound]\label{app_error}
    Let the classes of neural networks $\mathcal{F}_N$ be defined as in section \ref{sec_training} with depth $\mathcal{D}$, width $\mathcal{W}$ and bound $\mathcal{B}$, and let the excess risk $\mathcal{R}$ be defined as in (\ref{excess_risk}).
    Suppose Assumption (\ref{assump1}) holds with $B\le\mathcal{B}$. For NQ neural networks in $\mathcal{F}_N$, given any positive integers $U, M$, let the width $\mathcal{W}=38(K+1)(\lfloor\beta\rfloor+1)^2 d_1d_0^{\lfloor\beta\rfloor+1}U\log_2(8U)$ and depth $\mathcal{D}=21(\lfloor\beta\rfloor+1)^2d_0^{\lfloor\beta\rfloor+1}M\log_2(8M)$, then 
\begin{align}\notag
    \inf_{f\in\mathcal{F}_N}[\mathcal{R}(f)]&\le 18 (K+2)\mathcal{B}(\lfloor\beta\rfloor+1)^2 d_0^{\lfloor\beta\rfloor+1+(\beta\vee1)/2}(UM)^{-2\beta/d_0}+(K+2)\exp(-\mathcal{B})
\end{align}
where $d_0$ is the dimension of the input of NQ neural networks in $\mathcal{F}_N$.
\end{lemma}
The approximation error in Lemma \ref{app_error} is non-standard compared to existing results for quantile and robust regressions \citep{lederer2020risk,padilla2021adaptive,padilla2022quantile,shen2024nonparametric}. First, the approximation error is linear in $K$, the dimension of the NQ output, also the number of estimated quantile curves. Second, there is a $\exp(-\mathcal{B})$ error term since we use the truncation technique to deal with the unbounded preimage of ELU activation. The error incurred by the truncation decays exponentially fast with respect to $\mathcal{B}$, which can be neglected from the error analysis with a properly growing $\mathcal{B}$.

The approximation rate in Lemma \ref{app_error} can be further accelerated once the excess risk has a desirable local quadratic structure, as illustrated below.

\begin{assumption}[Local quadratic bound of the excess risk]
	\label{assump2}
There exist some constants $c^0=c^0(X,Y)>0$ and $\delta^0=\delta^0(X,Y)>0$ such that
	$$\mathcal{R}(f) -\mathcal{R}(Q_Y)\leq  \frac{c^0}{K}\sum_{k=1}^K \mathbb{E} \Vert f_{\tau_k}(X)-Q^{\tau_k}_Y(X) \Vert^2,$$
	for any $f=(f_{\tau_1},\ldots,f_{\tau_K})$ satisfying $\Vert f_{\tau_k}-Q_Y^{\tau_k} \Vert_{L^\infty(\mathcal{X}^0)}\leq \delta^0$ for $k=1,\ldots,K$, where $\mathcal{X}^0$ is any subset of $\mathcal{X}$ such that $\mathbb{P}(X\in\mathcal{X}^0)=\mathbb{P}(X\in\mathcal{X})$.
\end{assumption}

The technical assumption of a local quadratic structure for the excess risk can be satisfied when the density function of the conditional distribution $Y$ given $X$ has an upper bound near $Q_Y^{\tau_k}(X)$ for $k=1,\ldots, K$. With Assumption \ref{assump2}, we have an improved approximation error bound.

\begin{lemma}\label{app_error1}
    Suppose the conditions in Lemma \ref{app_error}  and Assumption \ref{assump2} hold. For NQ neural networks in $\mathcal{F}_N$, given any positive integers $U, M$, let the width $\mathcal{W}=38(K+1)(\lfloor\beta\rfloor+1)^2 d_1d_0^{\lfloor\beta\rfloor+1}U\log_2(8U)$ and depth $\mathcal{D}=21(\lfloor\beta\rfloor+1)^2d_0^{\lfloor\beta\rfloor+1}M\log_2(8M)$, then 
\begin{align}\notag
    \inf_{f\in\mathcal{F}_N}[\mathcal{R}(f)]&\le C(K+2)^2\left[\mathcal{B}^2(\lfloor\beta\rfloor+1)^4d_0^{2\lfloor\beta\rfloor+(\beta\vee 1)}(UM)^{-4\beta/d_0} + \exp(-2\mathcal{B})\right],
\end{align}
where $C>0$ is a universal constant and $d_0$ is the input dimension of NQ neural networks in $\mathcal{F}_N$.
\end{lemma} 
  



Based on the error decomposition in Lemma \ref{decomposition}, and our derived upper bounds for stochastic and approximation errors in Theorem \ref{sto_error} and Lemma \ref{app_error1}, we immediately obtain an upper bound for the excess risk $\mathcal{R}(\hat{f}_N)$ when the model is misspecified.

\begin{theorem}[Non-asymptotic Upper bounds]\label{nonasymp_error}
   Let the classes of neural networks $\mathcal{F}_N$ be defined as in section \ref{sec_training} with depth $\mathcal{D}$, width $\mathcal{W}$, size $\mathcal{S}$ and bound $\mathcal{B}$, and let the excess risk $\mathcal{R}$ be defined as in (\ref{excess_risk}).  Suppose Assumption (\ref{assump1}) holds with $B\le\mathcal{B}$ and Assumption \ref{assump2} holds. For NQ neural networks in $\mathcal{F}_N$, given any positive integers $U, M$, let the width $\mathcal{W}=38(K+1)(\lfloor\beta\rfloor+1)^2 d_1d_0^{\lfloor\beta\rfloor+1}U\log_2(8U)$ and depth $\mathcal{D}=21(\lfloor\beta\rfloor+1)^2d_0^{\lfloor\beta\rfloor+1}M\log_2(8M)$, then 
{\small
\begin{align*}
\mathbb{E}[\mathcal{R}(\hat{f}_N)]&\le C_1(K+2)^2\left[\mathcal{B}^2(\lfloor\beta\rfloor+1)^4d_0^{2\lfloor\beta\rfloor+(\beta\vee 1)}(UM)^{-4\beta/d_0} + \exp(-2\mathcal{B})\right]+C_2\cdot \frac{K\mathcal{B}^3\mathcal{S}\mathcal{D}\log(\mathcal{S})}{(\log N)^{-1}N}
\end{align*}
}
for $N\ge c\cdot\mathcal{D}\mathcal{S}\log(\mathcal{S})$ where $c,C_1,C_2>0$ are universal constants, and $d_0$ is the input dimension of the target quantile functions $Q_Y$.
\end{theorem}




The stochastic error is increasing in the network size while the approximation error is decreasing in its width and depth. To achieve the best possible convergence rate with respect to the sample size $N$, we need a balance between these two errors by finding a proper network architecture (width and depth). Note that the trade-off will heavily depend on the ratios $\beta/d_0$ where $\beta$ is the smoothness of the target functions $Q_Y$ and $d_0$ is the input dimension of $Q_Y$.



\begin{corollary}\label{cor1}
    Suppose the conditions in Theorem \ref{nonasymp_error} hold. Let $U=1$, $M=N^{d_0/[2(d_0+2\beta)]}$ and $\mathcal{B}=\log(N)$. Then the NQ net estimator $\hat{f}_N$ defined in (\ref{erm}) satisfies
\begin{align*}
  \mathbb{E}[\mathcal{R}(\hat{f}_N)]&\le
C\cdot K^2(\log N)^7 N^{-\frac{2\beta}{d_0+2\beta}}
\end{align*}
where $C>0$ is a constant depending only on $\beta$ and $d_0$.
\end{corollary}

Corrolary \ref{cor1} indicates that the excess risk of the NQ network estimator can achieve the minimax optimal rate (up to logarithms) for nonparametric regression \citep{stone1982optimal}.

\subsection{Curse of dimensionality}\label{sec_cod}

Recall that the excess risk bound in Corollary \ref{cor1} scales in a rate of $O(N^{-\frac{2\beta}{2\beta+d_0}})$ up to a logarithmic factor of $N$, where $N$ is the sample size, $\beta$ denotes the smoothness of the target function, and $d_0$ is the dimension of the covariate $X$. When the dimension of input $d_0$ is large, as in many machine learning tasks, the convergence rate of the NQ network estimator can be extremely slow. This is commonly referred to as the \emph{curse of dimensionality}. A slow convergence rate requires many more samples to attain a certain theoretical accuracy, which is usually impractical in real practice.

In modern statistics and machine learning tasks, many high-dimensional data tend to lie in the vicinity of a low-dimensional manifold \citep{carlsson2009topology,pope2021intrinsic}. This fact provides a way to mitigate the curse of dimensionality in the sense that the estimator maintains a desirable convergence rate even with a very large $d_0$. As in manifold learning \citep{fefferman2016testing} and semi-supervised learning \citep{belkin2004semi}, we posit the basic assumption of approximate low-dimensional manifold support below.

\begin{assumption}
	\label{low-dim}
	The covariate $X$ is supported on $\mathcal{M}_\rho$, a $\rho$-neighborhood of $\mathcal{M}\subset[0,1]^{d_0}$, where $\mathcal{M}$ is a compact $d_\mathcal{M}$-dimensional Riemannian sub-manifold and
	$$\mathcal{M}_\rho=\{x\in[0,1]^{d_0}: \inf\{\Vert x-y\Vert_2: y\in\mathcal{M}\}\leq \rho\}, \ \rho \in (0, 1).$$
\end{assumption}

With an approximate low-dimensional manifold support assumption, the approximation error for ReLU networks can be improved for nonparametric least squares regressions \citep{chen2019nonparametric,jiao2023deep}. Here we show that the low-dimensional manifold support assumption also results in a faster rate 
for the distributional estimation using NQ networks. %where the rate is in terms of the intrinsic dimension of the manifold.

\begin{lemma}[Approximation Error bound]\label{app_error_lowdim}
    Suppose Assumption \ref{assump1}, \ref{assump2}, \ref{low-dim} hold. Let the excess risk $\mathcal{R}$ be defined as in (\ref{excess_risk}) and $\mathcal{F}_N$ be defined as in section \ref{sec_training} with depth $\mathcal{D}$ and width $\mathcal{W}$. Given $\delta\in(0,1)$, let  the effective dimension $d_0^*=O(d_\mathcal{M}{\log(d_0/\delta)}/{\delta^2})$ be an integer such that $d_\mathcal{M}\leq d_0^*<d_0$. For any positive integers $U, M$, let $\mathcal{W}=38(\lfloor\beta\rfloor+1)^2 (K+1)(d_0^*)^{\lfloor\beta\rfloor+1}U\log_2(8U)$ and depth $\mathcal{D}=21(\lfloor\beta\rfloor+1)^2 (d_0^*)^{\lfloor\beta\rfloor+1}M\log_2(8M)$ for neural networks in $\mathcal{F}_N$, then 
    {\small
\begin{align*}
    \inf_{f\in\mathcal{F}_N}[\mathcal{R}(f)]&\le (18+C_2)^2(K+2)^2\mathcal{B}^2(\lfloor\beta\rfloor+1)^4(d_0^*)^{2\lfloor\beta\rfloor+(\beta\vee 1)}(UM)^{-4\beta/(d_0^*)}+(K+2)^2\exp(-2\mathcal{B}),
\end{align*}
}
when $\rho\leq C_2(UM)^{-2\beta/d_0^*}(\beta+1)^2(d_0^*)^{3\beta/2}\{(1-\delta)^{-1}\sqrt{{d_0}/{d_0^*}}+1\}^{-1}$ for some universal $C_2>0$.
\end{lemma}

    With Assumption \ref{low-dim}, the approximation error is improved in the exponent with the effective dimension $d_0^*$, which can be significantly smaller than the ambient dimension $d_0$ especially when the input dimension of data is high. %As a consequence, the approximation error for the base net will be dominated by the approximation error (\ref{app_error_R}) and (\ref{app_error_pi}) for R-Tower and T-tower.   
    If the data is assumed to have a low-dimensional structure, the rate of convergence derived in Corollary \ref{cor1} can also be improved. 

\begin{corollary}\label{cor2}
    Suppose the conditions in Theorem \ref{nonasymp_error} and Lemma \ref{app_error_lowdim} hold. Let $U=1$ and $M=N^{d_0^*/[2(d_0^*+2\beta)]}$. Then the NQ net estimator $\hat{f}_N$ defined in (\ref{erm}) satisfies
\begin{align*}
  \mathbb{E}[\mathcal{R}(\hat{f}_N)]&\le
C\cdot K^2(\log N)^7 N^{-\frac{2\beta}{d_0^*+2\beta}}
\end{align*}
where $C>0$ is a constant depending only on $\beta$, $d_0$ and $d_0^*$.
\end{corollary}




